On the adaptation of context-aware services

Ubiquitous networking empowered by Beyond 3G networking makes it possible for mobile users to access networked software services across heterogeneous infrastructures by resource-constrained devices. Heterogeneity and device limitedness creates serious problems for the development and deployment of mobile services that are able to run properly on the execution context and are able to ensures that users experience the "best" Quality of Service possible according to their needs and specific contexts of use. To face these problems the concept of adaptable service is increasingly emerging in the software community. In this paper we describe how CHAMELEON, a declarative framework for tailoring adaptable services, is used within the IST PLASTIC project whose goal is the rapid and easy development/deployment of self-adapting services for B3G networks.

==> introduction_old.tex <==
\section{Introduction}
\label{sec:introduction}
	introduction here.
	
	#####
	Scaletta:
	1. introduction (Plastic Development Process con focus su adattamento)
	2. dove l'adattamento si inserisce nel processo di service deployment dell'applicazione (figura triangolare : discovery, .....)
	3. cosa si intende per contesto
	4. strategie di adattamento (come scegliamo)
	5. programming model
	6. conclusioni

	
	Paola: specificare dove si inserisce l'adattamento subito prima di stringere la SLA.
	evidenziare che l'adattamento non avviene solo in base alla caratteristiche del device 
, ma tiene anche conto del presunto pattern di mobilita'.		 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ffaa"
%%% End:

